Implementing Communication-Optimal Parallel and Sequential QR Factorizations

We present parallel and sequential dense QR factorization algorithms for tall and skinny matrices and general rectangular matrices that both minimize communication, and are as stable as Householder QR. The sequential and parallel algorithms for tall and skinny matrices lead to significant speedups in practice over some of the existing algorithms, including LAPACK and ScaLAPACK, for example up to 6.7x over ScaLAPACK. The parallel algorithm for general rectangular matrices is estimated to show significant speedups over ScaLAPACK, up to 22x over ScaLAPACK.

==> platforms.tex <==
\section{Platforms of interest for TSQR experiments and models}\label{S:TSQR:platforms}

\subsection{A large, but composable tuning space}

TSQR is not a single algorithm, but a space of possible algorithms.
It encompasses all possible reduction tree shapes, including:
\begin{enumerate}
  \item Binary (to minimize number of messages in the parallel case)
  \item Flat (to minimize communication volume in the sequential
    case)
  \item Hybrid (to account for network topology, and/or to balance
    bandwidth demands with maximum parallelism)
\end{enumerate}
as well as all possible ways to perform the local QR factorizations,
including:
\begin{enumerate}
  \item (Possibly multithreaded) standard LAPACK (DGEQRF)
  \item An existing parallel QR factorization, such as ScaLAPACK's
    PDGEQRF 
  \item A ``divide-and-conquer'' QR factorization (e.g.,
    \cite{elmroth1998new})
  \item Recursive (invoke another form of TSQR)
\end{enumerate}
Choosing the right combination of parameters can help minimize
communication between any or all of the levels of the memory
hierarchy, from cache and shared-memory bus, to DRAM and local disk,
to parallel filesystem and distributed-memory network interconnects,
to wide-area networks.

The huge tuning space makes it a challenge to pick the right platforms
for experiments.  Luckily, TSQR's hierarchical structure makes tunings
\emph{composable}.  For example, once we have a good choice of
parameters for TSQR on a single multicore node, we don't need to
change them when we tune TSQR for a cluster of these nodes.  From the
cluster perspective, it's as if the performance of the individual
nodes improved.  This means that we can benchmark TSQR on a small,
carefully chosen set of scenarios, with confidence that they represent
many platforms of interest.


\subsection{Platforms of  interest}\label{SS:TSQR:platforms:interest}
\label{TSQR:perfres:platforms-of-interest}

Here we survey a wide variety of interesting platforms for TSQR, and
explain the key features of each that we will distill into a small
collection of experiments.

\subsubsection{Single-node parallel, and explicitly swapping}

The ``cluster of shared-memory parallel (SMP) nodes'' continues to
provide a good price-performance point for many large-scale
applications.  This alone would justify optimizing the single-node
case.  Perhaps more importantly, the ``multicore revolution'' seeks to
push traditionally HPC applications into wider markets, which favor
the single-node workstation or even the laptop over the expensive,
power-hungry, space-consuming, difficult-to-maintain cluster.  A large
and expanding class of users may never run their jobs on a cluster.

%
% mfh 25 Jan 2008:
% FIXME: some of this (e.g., definition of ``explicitly swapping'')
% should go in the Introduction (???).
%
Multicore SMPs can help reduce communication costs, but cannot
eliminate them.  TSQR can exploit locality by sizing individual
subproblems to fit within any level of the memory hierarchy.  This
gives programmers explicit control over management of communication
between levels, much like a traditional ``out-of-core''
algorithm.\footnote{We avoid this label because it's an anachronism
  (``core'' refers to main system memory, constructed of solenoids
  rather than transistors or DRAM), and because people now easily
  confuse ``core'' with ``processing unit'' (in the sense of
  ``multicore'').  We prefer the more precise term \emph{explicitly
    swapping}, or ``out-of-X'' for a memory hierarchy level X.  For
  example, ``out-of-DRAM'' means using a disk, flash drive, or other
  storage device as swap space for problems too large to solve in
  DRAM.}  TSQR's hierarchical structure makes explicit swap management
easy; it's just another form of communication.  It gives us an
optimized implementation for ``free'' on platforms like Cell or GPUs,
which require explicitly moving data into separate storage areas for
processing.  Also, it lets us easily and efficiently solve problems
too large to fit in DRAM.  This seems like an old-fashioned issue,
since an individual node nowadays can accommodate as much as 16 GB of
DRAM.  Explicitly swapping variants of libraries like ScaLAPACK tend
to be ill-maintained, due to lack of interest.  However, we predict a
resurgence of interest in explicitly-swapping algorithms, for the
following reasons:
\begin{itemize}
  \item Single-node workstations will become more popular than
    multinode clusters, as the number of cores per node increases.

  \item The amount of DRAM per node cannot scale linearly with the
    number of cores per node, because of DRAM's power requirements.
    Trying to scale DRAM will wipe out the power savings promised by
    multicore parallelism.  % e.g., Sam's Niagra 2 box takes 600+ W
                            % with 16 GB of DRAM, despite the Niagra
                            % project's promise of lower power.
  \item The rise to prominence of mobile computing -- e.g., more
    laptops than desktops were sold in U.S.\ retail in 2006 --
    drives increasing concern for total-system power use.

  \item Most operating systems do not treat ``virtual memory'' as
    another level of the memory hierarchy.  Default and recommended
    configurations for Linux, Windows XP, Solaris, and AIX on modern
    machines assign only 1--3 times as much swap space as DRAM, so
    it's not accurate to think of DRAM as a cache for disk.  Few
    operating systems expand swap space on demand, and expanding it
    manually generally requires administrative access to the machine.
    It's better for security and usability to ask applications to adapt
    to the machine settings, rather than force users to change their
    machine for their applications.

  \item \emph{Unexpected} use of virtual memory swap space generally
    slows down applications by orders of magnitude.  HPC programmers
    running batch jobs consider this a performance problem serious
    enough to warrant terminating the job early and sizing down the
    problem.  Users of interactive systems typically experience large
    (and often frustrating) delays in whole-system responsiveness when
    extensive swapping occurs.
%%     This causes a lot of frustration and dissatisfaction, as
%%     suggested by the nicknames they attach to GUI indicators of
%%     unresponsiveness (e.g., ``Hourglass of Pain'' or ``Spinning Beach
%%     Ball of Death'').

  \item In practice, a single application need not consume all memory
    in order to trigger the virtual memory system to swap extensively.

  \item Explicitly swapping software does not stress the OS's virtual
    memory system, and can control the amount of memory and disk
    bandwidth resources that it uses.

  \item Alternate storage media such as solid-state drives offer more
    bandwidth than traditional magnetic hard disks.  Typical hard disk
    read or write bandwidth as of this work's publication date is
    around 60 MB/s, whereas Samsung announced in May 2008 the upcoming
    release of a 256 GB capacity solid-state drive with 200 MB/s read
    bandwidth and 160 MB/s write bandwidth \cite{samsung2008ssd}.
    Solid-state drives are finding increasing use in mobile devices
    and laptops, due to their lower power requirements.  This will
    make out-of-DRAM applications more attractive by widening any
    bandwidth bottlenecks.
\end{itemize}


\subsubsection{Distributed-memory machines}

Avoiding communication is a performance-enhancing strategy for
distributed-memory architectures as well.  TSQR can improve
performance on traditional clusters as well as other networked
systems, such as grid and perhaps even volunteer computing.  Avoiding
communication also makes improving network reliability less of a
performance burden, as software-based reliability schemes use some
combination of redundant and/or longer messages.  Many
distributed-memory supercomputers have high-performance parallel
filesystems, which increase the bandwidth available for out-of-DRAM
TSQR.  This enables reducing per-node memory requirements without
increasing the number of nodes needed to solve the problem.


\subsection{Pruning the platform space}\label{SS:TSQR:platforms:pruning}

For single-node platforms, we think it pays to investigate both
problems that fit in DRAM (perhaps with explicit cache management),
and problems too large to fit in DRAM, that call for explicit swapping
to a local disk.  High-performance parallel filesystems offer
potentially much more bandwidth, but we chose not to use them for our
experiments for the following reasons:
\begin{itemize}
  \item Lack of availability of a single-node machine with exclusive
    access to a parallel filesystem
  \item On clusters, parallel filesystems are usually shared among all
    cluster users, which would make it difficult to collect repeatable
    timings.
\end{itemize}
For multinode benchmarks, we opted for traditional clusters rather
than volunteer computing, due to the difficulty of obtaining
repeatable timings in the latter case.



\subsection{Platforms for experiments}\label{SS:TSQR:platforms:exp}


We selected the following experiments as characteristic of the space
of platforms:
\begin{itemize}
\item Single node, sequential, out-of-DRAM, and
\item Distributed memory, in-DRAM on each node.
\end{itemize}

We ran sequential TSQR on a laptop with a single PowerPC CPU.  It
represents the embedded and mobile space, with its tighter power and
heat requirements.  Details of the platform are as follows:
\begin{itemize}
\item Single-core PowerPC G4 (1.5 GHz) 
\item 512 KB of L2 cache
\item 512 MB of DRAM on a 167 MHz bus
\item One Fujitsu MHT2080AH 80 HB hard drive (5400 RPM) 
\item MacOS X 10.4.11
\item GNU C Compiler (gcc), version 4.0.1
\item vecLib (Apple's optimized dense linear algebra library),
  version 3.2.2
\end{itemize}
%   \item[Clovertown]
%     \begin{itemize}
%     \item Dual-socket Intel Clovertown (model E5345, 2.33 GHz, four
%     cores per socket) 
%     \item Two L2 caches of 4MB each, one for each of
%     the two pairs of cores on a socket  
%     \item 16 GB of DRAM
%     \item One 300 GB 10K RPM local disk with maximum sustained
%       bandwidth of 89 GB/s
%     \item Debian Linux (kernel version 2.6.18), with virtual memory
%       overcommit enabled
%     \item Intel C Compiler (icc), version 10.0
%     \item Intel Math Kernel library (multithreaded BLAS and LAPACK),
%       version 9.1.023
%     \end{itemize}

We ran parallel TSQR on the following distributed-memory machines:
\begin{enumerate}
\item Pentium III cluster (``Beowulf'')
\begin{itemize}
\item Operated by the University of Colorado at Denver and the Health
  Sciences Center
\item 35 dual-socket 900 MHz Pentium III nodes with Dolphin
  interconnect
\item Floating-point rate:  900 Mflop/s per processor, peak
\item Network latency: less than 2.7 $\mu$s, benchmarked\footnote{See
  \url{http://www.dolphinics.com/products/benchmarks.html}.}
\item Network bandwidth: 350 MB/s, benchmarked upper bound
% \item MPICH (MPI implementation) v.\ 2.1
% \item Kazushige Goto's optimized BLAS implementation, v.\ 1.10
% \item LAPACK 3.1.1
\end{itemize}

\item IBM BlueGene/L (``Frost'')
\begin{itemize}
\item Operated by the National Center for Atmospheric Research
\item One BlueGene/L rack with 1024 700 MHz compute CPUs
\item Floating-point rate:  2.8 Gflop/s per processor, peak
\item Network\footnote{The BlueGene/L has two separate networks -- a
    torus for nearest-neighbor communication and a tree for
    collectives.  The latency and bandwidth figures here are for the
    collectives network.} latency:  1.5 $\mu$s, hardware
\item Network one-way bandwidth:  350 MB/s, hardware
\end{itemize}
\end{enumerate}



\subsection{Platforms for performance models}\label{SS:TSQR:platforms:models}

In Section \ref{S:CAQR:perfest}, we estimate performance of CAQR, our
QR factorization algorithm on a 2-D matrix layout, on three different
parallel machines: an existing IBM POWER5 cluster with a total of 888
processors (``IBM POWER5''), a future proposed petascale machine with
8192 processors (``Peta''), and a collection of 128 processors linked
together by the Internet (``Grid'').  Here are the parameters we use
in our models for the three parallel machines:
\begin{itemize}
\item IBM POWER5
\begin{itemize}
  \item 888 processors
  \item Floating-point rate:  7.6 Gflop/s per processor, peak
  \item Network latency:  5 $\mu$s
  \item Network bandwidth:  3.2 GB/s
\end{itemize}

\item Peta
\begin{itemize}
  \item 8192 processors
  \item Floating-point rate:  500 Gflop/s per processor, peak
  \item Network latency:  10 $\mu$s
  \item Network bandwidth:  4 GB/s
\end{itemize}

\item Grid
\begin{itemize}
  \item 128 processors
  \item Floating-point rate:  10 Tflop/s, peak
  \item Network latency:  0.1 s
  \item Network bandwidth:  0.32 GB/s
\end{itemize}
\end{itemize}
Peta is our projection of a future high-performance computing cluster,
and Grid is our projection of a collection of geographically separated
high-performance clusters, linked over a TeraGrid-like backbone.  Each
``processor'' of Peta may itself be a parallel multicore node, but we
consider it as a single fast sequential processor for the sake of our
model.  Similarly, each ``processor'' of Grid is itself a cluster, but
we consider it as a single very fast sequential processor.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> pr-tsqr-algorithm.tex <==
\section{TSQR as a reduction}
\label{pr:reduction}

\subsection{Optimizing local factorizations in TSQR}
\label{pr:TSQR_localopt} 

Most of the QR factorizations performed during TSQR involve matrices
consisting of one or more triangular factors stacked atop one another.
We can ignore this zero structure and still get a correct
factorization, but if we do we will do several times as many floating
point operations as necessary (up to 5$\times$ in the parallel case
and 2$\times$ in the sequential case). Previous authors have suggested
using Givens rotations to avoid this \cite{pothen1989distributed}, but
this would make it hard to achieve BLAS3 performance.

Our observation is that not only is it possible to used blocked
Householder transformations that both do minimal arithmetic and permit
BLAS3 performance, but in fact we can organize the algorithm to get
{\em better} BLAS3 performance than conventional QR decomposition.
The empirical data justifying this claim appears elsewhere
(\cite[Section 12]{TSQR_technical_report}), but we outline the
algorithm here.

We illustrate with the QR decomposition of a pair $[R_0 ; R_1 ]$ of
5-by-5 triangular matrices.  Their sparsity pattern, and that of the
Householder vectors from their QR decomposition are shown below:

\begin{equation}\label{eq:fact_2rs}
\begin{pmatrix}
R_0 \\
R_1\\
\end{pmatrix}
=
\begin{pmatrix}
x & x & x & x & x \\
  & x & x & x & x \\
  &   & x & x & x \\
  &   &   & x & x \\
  &   &   &   & x \\
x & x & x & x & x \\
  & x & x & x & x \\
  &   & x & x & x \\
  &   &   & x & x \\
  &   &   &   & x \\
\end{pmatrix}
\Longrightarrow
{\rm Householder} = 
\begin{pmatrix}
1 &   &   &   &   \\
  & 1 &   &   &   \\
  &   & 1 &   &   \\
  &   &   & 1 &   \\
  &   &   &   & 1 \\
x & x & x & x & x  \\
  & x & x & x & x \\
  &   & x & x & x \\
  &   &   & x & x \\
  &   &   &   & x \\
\end{pmatrix}.
\end{equation}

This picture suggests that it is straightforward to adapt both the
unblocked Householder decomposition and its blocked version in
\cite{schreiber1989storage}, by storing the Householder vectors on top
of the zeroed-out entries as usual, and simply by changing the lengths
of the vectors involved in updates of the trailing matrix.  For the
case of two $n$-by-$n$ triangular matrices, exploiting this structure
lowers the operation count to $\frac{2}{3}n^3$ from about
$\frac{10}{3}n^3$.  It is also possible to do this when $q$ triangles
are stacked atop one another, generating $(q-1)n(n+1)/2$ parameters.
See \cite[Section 6]{TSQR_technical_report}) for details.

Most importantly, we can apply Elmroth and Gustavson's recursive QR
algorithm \cite{elmroth2000applying} to the matrices in fast memory
(in the sequential case) or local processor memory (in the parallel
case). Various authors have observed that Elmroth's and Gustavson's
algorithm works well on tall-skinny matrices, but this applies only if
the data fits in fast (or local) memory, which is what we can
guarantee.

